You Truly Understand What I Need: Intellectual and Friendly Dialogue Agents grounding Knowledge and Persona

To build a conversational agent that interacts fluently with humans, previous studies blend knowledge or personal profile into the pre-trained language model. However, the model that considers knowledge and persona at the same time is still limited, leading to hallucination and a passive way of using personas. We propose an effective dialogue agent that grounds external knowledge and persona simultaneously. The agent selects the proper knowledge and persona to use for generating the answers with our candidate scoring implemented with a poly-encoder. Then, our model generates the utterance with lesser hallucination and more engagingness utilizing retrieval augmented generation with knowledge-persona enhanced query. We conduct experiments on the persona-knowledge chat and achieve state-of-the-art performance in grounding and generation tasks on the automatic metrics. Moreover, we validate the answers from the models regarding hallucination and engagingness through human evaluation and qualitative results. We show our retriever's effectiveness in extracting relevant documents compared to the other previous retrievers, along with the comparison of multiple candidate scoring methods. Code is available at https://github.com/dlawjddn803/INFO

==> figures/humaneval.tex <==
\section{Human Evaluation Distribution on Each Criteria} \label{sec:humaneval_dist}


\begin{figure}[ht]
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/graph_adequate.png}
\caption{Adequacy}
\label{fig:human_a}
\end{subfigure}\hfill
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/graph_fluent.png}
\caption{Fluency}
\label{fig:human_f}
\end{subfigure}%
\caption{The distribution of the rank on the adequacy and fluency criteria. Guide A to E indicates INFO, BART$_{base}$, BART$_{large}$, GPT-2$_{small}$, and GPT-2$_{medium}$, in the order.}
\label{fig:human_af}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/graph_adequate.png}
\caption{Provenance}
\label{fig:human_p}
\end{subfigure}\hfill
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/graph_persona.png}
\caption{Engagingness}
\label{fig:human_e}
\end{subfigure}%
\caption{The distribution of the rank on the provenance and engagingness criteria. Guide A to E indicates INFO, BART$_{base}$, BART$_{large}$, GPT-2$_{small}$, and GPT-2$_{medium}$, in the order.}
\label{fig:human_pe}
\end{figure}


\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/graph_hallucination.png}
\caption{The distribution of the rank on the less hallucination criterion. Note that the highest rank (1) means the most hallucinated. Guide A to E indicates INFO, BART$_{base}$, BART$_{large}$, GPT-2$_{small}$, and GPT-2$_{medium}$, in the order. } \label{fig:human_h}
\end{figure*}


==> figures/overview.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/overview.png}
\caption{Overview of our method. $U$ is the input comprises dialogue history and knowledge snippet, and $cand$ denotes each candidate from the grounding tasks. The grounding score is obtained through the dot product operation with the representation of input context $U_{dial}$ and candidate $a_{t}$. The predicted sources convert into the knowledge-persona enhanced query (KPEQ) with dialogue history and KPEQ is fed into the retrieval-augmented generator to generate the responses.} \label{fig:overview}
\end{figure*}

